Competitions in AI -- Robustly Ranking Solvers Using Statistical Resampling

Solver competitions play a prominent role in assessing and advancing the state of the art for solving many problems in AI and beyond. Notably, in many areas of AI, competitions have had substantial impact in guiding research and applications for many years, and for a solver to be ranked highly in a competition carries considerable weight. But to which extent can we expect competition results to generalise to sets of problem instances different from those used in a particular competition? This is the question we investigate here, using statistical resampling techniques. We show that the rankings resulting from the standard interpretation of competition results can be very sensitive to even minor changes in the benchmark instance set used as the basis for assessment and can therefore not be expected to carry over to other samples from the same underlying instance distribution. To address this problem, we introduce a novel approach to statistically meaningful analysis of competition results based on resampling performance data. Our approach produces confidence intervals of competition scores as well as statistically robust solver rankings with bounded error. Applied to recent SAT, AI planning and computer vision competitions, our analysis reveals frequent statistical ties in solver performance as well as some inversions of ranks compared to the official results based on simple scoring.

==> tables/imagenet/object-classification-additional-data/ilsvrc2015_object_classification_additional_data_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 1    & Amax 6 (1) \\
     2 & 2    & Trimps-Soushen 9 (2) \\
     3 & 3.5  & CUImage 8 (3), CUImage 7 (3) \\


==> tables/imagenet/object-classification-provided-data/ilsvrc2015_object_classification_provided_data_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 2    & MSRA 7 (1), MSRA 6 (1), ReCeption 6 (3) \\
     2 & 4    & MSRA 8 (4) \\
     3 & 5    & Trimps-Soushen 7 (5) \\
     4 & 6.5    & Trimps-Soushen 8 (6), Trimps-Soushen 6 (6) \\
     5 & 9    & Trimps-Soushen 10 (8), Qualcomm Research 8 (9), Qualcomm Research 7 (10) \\
     6 & 12.5    & VUNO 7 (11), VUNO 6 (11), Qualcomm Research 6 (13), Qualcomm Research 9 (13) \\
     7 & 15.5    & CIL 7 (15), CIL 6 (15) \\
     8 & 17.5    & cuhk loc 7 (17), CUImage 6 (17) \\
     9 & 19.5    & MCG-ICT-CAS 10 (19), MCG-ICT-CAS 9 (20) \\
    10 & 22    & MCG-ICT-CAS 8 (21), MCG-ICT-CAS 7 (21), HiVision 6 (23) \\
    11 & 24    & MCG-ICT-CAS 6 (24) \\
    12 & 25    & Szokcka Research Group 7 (25) \\
    13 & 27.5    & JHL 7 (26), Lunit-KAIST 6 (27), KAISTNIA ETRI 7 (28), KAISTNIA ETRI 6 (29) \\
    14 & 35    & Lunit-KAIST 7 (30), Szokcka Research Group 6 (31), KAISTNIA ETRI 10 (33), \\
       &       & KAISTNIA ETRI 8 (33), KAISTNIA ETRI 9 (33), CIL 8 (35), CIL 10 (36), CIL 9 (38), \\
       &       & FACEALL-BUPT 6 (40), FACEALL-BUPT 7 (40), FACEALL-BUPT 8 (40) \\
    15 & 41    & Lunit-KAIST 8 (37) \\
    16 & 42    & Lunit-KAIST 9 (42) \\
    17 & 43.5    & MIPAL SNU 6 (43), MIPAL SNU 7 (43) \\
    18 & 46.5    & bioinf@JKU 7 (46), bioinf@JKU 8 (46), bioinf@JKU 9 (46), bioinf@JKU 6 (46) \\
    19 & 49    & Tencent-Bestimage 7 (49) \\
    20 & 51    & Tencent-Bestimage 9 (50), Tencent-Bestimage 8 (51), Deep Punx 6 (52) \\
    21 & 53.5    & ITU 6 (53), Miletos 6 (53) \\
    22 & 55    & PCL Bangalore 6 (55) \\
    23 & 56    & APL 7 (56) \\
    24 & 57.5    & DIT TITECH 6 (57), Tencent-Bestimage 6 (58) \\
    25 & 59    & Deep Punx 8 (59) \\
    26 & 60    & Deep Punx 7 (60) \\
    27 & 61    & JHL 6 (61) \\
    28 & 62    & APL 6 (62) \\


==> tables/imagenet/object-detection-additional-data/ilsvrc2015_object_detection_additional_data_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 1    & Amax 2 (1) \\
     2 & 2    & Amax 1 (2) \\
     3 & 3    & CUImage 2 (3) \\
     4 & 4    & MIL-UT 1 (4) \\
     5 & 5    & MIL-UT 2 (5) \\
     6 & 6    & Trimps-Soushen 1 (6) \\
     7 & 7.5    & Trimps-Fudan-HUST 1 (7), Trimps-Soushen 3 (8) \\
     8 & 9    & Futurecrew 2 (9) \\
     9 & 10    & Futurecrew 3 (10) \\
    10 & 11    & Futurecrew 1 (11) \\
    11 & 12    & 1-HKUST 1 (12) \\
    12 & 13    & 1-HKUST 2 (13) \\


==> tables/imagenet/object-detection-provided-data/ilsvrc2015_object_detection_provided_data_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 1    & MSRA 1 (1) \\
     2 & 2    & Qualcomm Research 1 (2) \\
     3 & 3    & CUImage 1 (3) \\
     4 & 4    & The University of Adelaide 1 (4) \\
     5 & 6.5    & MCG-ICT-CAS 3 (5), MCG-ICT-CAS 5 (6), MCG-ICT-CAS 4 (7), DROPLET-CASIA 2 (8) \\
     6 & 10.5    & Trimps-Soushen 2 (9), MCG-ICT-CAS 2 (10), DROPLET-CASIA 1 (11), MCG-ICT-CAS 1 (12) \\
     7 & 13.5    & Yunxiao 1 (13), Trimps-Fudan-HUST 2 (14) \\
     8 & 15    & HiVision 1 (15) \\
     9 & 16    & SYSU Vision 3 (16) \\
    10 & 17    & SYSU Vision 2 (17) \\
    11 & 18    & FACEALL-BUPT 4 (18) \\
    12 & 19    & FACEALL-BUPT 3 (19) \\
    13 & 22    & DEEPimagine 4 (20), SYSU Vision 1 (21), DEEPimagine 3 (22), ITLab - Inha 2 (24), ITLab - Inha 1 (25) \\
    14 & 25    & DEEPimagine 2 (23) \\
    15 & 28    & ITLab - Inha 5 (26), ITLab - Inha 3 (27), DEEPimagine 1 (28), DEEPimagine 5 (29), FACEALL-BUPT 1 (30) \\
    16 & 31.5    & ITLab - Inha 4 (31), FACEALL-BUPT 2 (32) \\
    17 & 33    & JHL 1 (33) \\
    18 & 34    & USTC UBRI 1 (34) \\
    19 & 35    & hustvision 1 (35) \\
    20 & 37    & darkensemble 1 (36), ESOGU MLCV 1 (37), ESOGU MLCV 2 (38) \\
    21 & 39    & N-ODG 1 (39) \\


==> tables/imagenet/object-detection-video-additional-data/ilsvrc2015_object_detection_video_additional_data_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 1.5    & Amax 11 (1), CUVideo 12 (2) \\
     2 & 3.5    & Trimps-Soushen 13 (3), Trimps-Soushen 14 (4) \\
     3 & 5    & BAD 14 (5) \\
     4 & 7    & BAD 12 (6), BAD 13 (7), BAD 11 (8) \\
     5 & 9.5    & BAD 15 (9), NECLAMA 11 (10) \\


==> tables/imagenet/object-detection-video-provided-data/ilsvrc2015_object_detection_video_provided_data_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 1    & CUVideo 11 (1) \\
     2 & 4    & ITLab VID - Inha 13 (2), ITLab VID - Inha 12 (3), UIUC-IFP 11 (6), UIUC-IFP 12 (6), UIUC-IFP 13 (6) \\
     3 & 7    & ITLab VID - Inha 11 (4) \\
     4 & 11    & Trimps-Soushen 11 (8), Trimps-Soushen 12 (9), UIUC-IFP 14 (10), 1-HKUST 14 (11), 1-HKUST 13 (12), \\
       &       & 1-HKUST 15 (13), RUC BDAI 11 (17) \\
     5 & 16    & HiVision 12 (14), 1-HKUST 12 (15), 1-HKUST 11 (16) \\
     6 & 19    & NICAL 11 (18), FACEALL-BUPT 13 (19), FACEALL-BUPT 12 (20) \\
     7 & 21.5    & FACEALL-BUPT 11 (21), MPG UT 11 (22) \\
     8 & 23    & ART Vision 12 (23) \\


==> tables/imagenet/object-localization-additional-data/ilsvrc2015_object_localization_additional_data_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 1    & Trimps-Soushen 9 (1) \\
     2 & 2    & Amax 6 (2) \\
     3 & 3    & CUImage 7 (3) \\
     4 & 4    & CUImage 8 (4) \\


==> tables/imagenet/object-localization-provided-data/ilsvrc2015_object_localization_provided_data_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 &  1.5  & MSRA 6 (1), MSRA 7 (2) \\
     2 &  3    & MSRA 8 (3) \\
     3 &  5    & Trimps-Soushen 8 (4), Qualcomm Research 8 (5), Qualcomm Research 7 (6) \\
     4 &  8    & Qualcomm Research 6 (7), Trimps-Soushen 7 (8), Trimps-Soushen 10 (9) \\
     5 & 10    & Trimps-Soushen 6 (10) \\
     6 & 13    & Lunit-KAIST 9 (11), MCG-ICT-CAS 10 (12), MCG-ICT-CAS 8 (13), MCG-ICT-CAS 9 (14), MCG-ICT-CAS 7 (16) \\
     7 & 16    & Lunit-KAIST 8 (15) \\
     8 & 17    & Lunit-KAIST 7 (17) \\
     9 & 19.5  & Tencent-Bestimage 9 (18), Tencent-Bestimage 8 (19), Qualcomm Research 9 (20), MCG-ICT-CAS 6 (21) \\
    10 & 22.5  & Lunit-KAIST 6 (22), Tencent-Bestimage 7 (23) \\
    11 & 25    & Tencent-Bestimage 6 (24), ReCeption 6 (25), cuhk loc 7 (26) \\
    12 & 27    & CUImage 6 (27) \\
    13 & 28.5  & CIL 10 (28), CIL 9 (30) \\
    14 & 30    & CIL 8 (29) \\
    15 & 31.5  & VUNO 6 (31), VUNO 7 (32) \\
    16 & 33    & CIL 7 (33) \\
    17 & 34    & CIL 6 (34) \\
    18 & 37    & KAISTNIA ETRI 7 (35), KAISTNIA ETRI 10 (36), KAISTNIA ETRI 9 (37), KAISTNIA ETRI 8 (38), HiVision 6 (40) \\
    19 & 40    & KAISTNIA ETRI 6 (39) \\
    20 & 41    & FACEALL-BUPT 8 (41) \\
    21 & 43    & MIPAL SNU 7 (42), FACEALL-BUPT 7 (43), FACEALL-BUPT 6 (44) \\
    22 & 45    & MIPAL SNU 6 (45) \\
    23 & 46    & PCL Bangalore 6 (46) \\
    24 & 47    & bioinf@JKU 8 (47) \\
    25 & 48    & bioinf@JKU 7 (48) \\
    26 & 49.5  & Szokcka Research Group 7 (49), Szokcka Research Group 6 (50) \\
    27 & 51.5  & ITU 6 (51), Miletos 6 (51) \\
    28 & 53    & JHL 7 (53) \\
    29 & 54.5  & APL 7 (54), Deep Punx 6 (55) \\
    30 & 56.5  & bioinf@JKU 6 (56), bioinf@JKU 9 (57) \\
    31 & 58    & DIT TITECH 6 (58) \\
    32 & 59    & Deep Punx 7 (59) \\
    33 & 60    & JHL 6 (60) \\
    34 & 61    & Deep Punx 8 (61) \\
    35 & 62    & APL 6 (62) \\


==> tables/ipc/seq-agl/ipc2014_seq_agl_domain_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 1      & YAHSP3 (1) \\
     2 & 4.5    & Madagascar-pC (2), Madagascar (3), PROBE (4), BFS(f) (5), Fast Downward Cedalion (6), Freelunch (7) \\
     3 & 9      & YAHSP3-MT (8), ArvandHerd (9), IBaCoP (10) \\
     4 & 11.5   & USE (11), Jasper (12) \\
     5 & 14     & SIW (13), mercury (14), IBaCoP2 (15) \\


==> tables/ipc/seq-opt/ipc2014_seq_opt_domain_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 1    & SymBA*-2 (1) \\
     2 & 2    & SymBA*-1 (2) \\
     3 & 4    & cGamer (3), SPM\&S (4), RIDA (5) \\
     4 & 8.5  & Dynamic-Gamer (6), AllPACA (7), Fast Downward Cedalion (8), Metis (9), NuCeLaR (10), Rational Lazy A* (11) \\
     5 & 12   & Gamer (12) \\
     6 & 14   & hflow (13), MIPlan (14), DPMPlan (15) \\
     7 & 16.5 & h++-ce (16), h++ (17) \\


==> tables/ipc/seq-sat/ipc2014_seq_sat_domain_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 1.5    & IBaCoP2 (1), IBaCoP (2) \\
     2 & 4.5    & Mercury (3), MIPlan (4), Jasper (5), Fast Downward Uniform (6) \\
     3 & 8      & Fast Downward Cedalion (7), ArvandHerd (8), Fast Downward Stone Soup 2014 (9) \\
     4 & 10     & DPMPlan (10) \\
     5 & 12.5   & USE (11), NuCeLaR (12), RPT (13), BFS(f) (14) \\
     6 & 15     & BiFD (15) \\
     7 & 17     & DAE-YAHSP (16), Freelunch (17), YAHSP3-MT (18) \\
     8 & 19     & YAHSP3 (19) \\
     9 & 20     & Planets (20) \\


==> tables/sat/agile/sat2016_agile_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
1   & 1      & Riss6 default (1) \\
2   & 3.5    & tb\_glucose\_agile default (2), CHBR\_glucose\_agile default (3), \\
    &        & CHBR\_glucose\_tuned\_agile default (4), glue\_alt default (6) \\
3   & 6      & tc\_glucose\_agile default (5) \\
4   & 8      & glucosePLE default (7), glucose\_hack\_kiel\_newScript default (8), \\
    &        & glucose\_hack\_kiel\_newScript hack\_configuration (9) \\
5   & 11     & abcdSAT\_drup default (10), glucose\_hack\_kiel\_newScript main\_new (11), \\
    &        & glueminisat-2.2.10-81-agile agile (12) \\
6   & 14.5   & Riss6 noPP (13), gulch-agile default (14), MapleCOMSPS\_CHB\_no\_DRUP CHB\_VSIDS\_no\_drup (15), \\
    &        & gulch-once default (16) \\
7   & 17.5   & MapleGlucose default (17), Riss6 blackbox (18) \\
8   & 21     & GHackCOMSPS\_no\_DRUP ghack (19), MapleCOMSPS\_LRB\_no\_DRUP LRB\_VSIDS\_no\_drup (20), \\
    &        & cmsat5\_agile2 default (21), MapleCOMSPS\_no\_DRUP seq\_LRB\_VSIDS\_no\_drup (22), \\
    &        & COMiniSatPS Chandrasekhar no DRUP no\_drup (23) \\
9   & 24.5   & splatz default (24), MapleCMS default (25) \\
10  & 26     & lingeling default (26) \\


==> tables/sat/main-application/sat2016_main_application_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
1    & 14    & MapleCOMSPS\_LRB\_DRUP LRB\_VSIDS\_drup (1), MapleCOMSPS\_DRUP seq\_LRB\_VSIDS\_drup (2), \\
     &       & CHBR\_glucose default (3), CHBR\_glucose\_tuned default (4), glucose default (4), \\
     &       & abcdSAT\_drup default (6), MapleCMS default (6), Beans And Eggs default (10), \\
     &       & cmsat5\_autotune2 default (10), Riss6 blackbox\_DRAT (10), Lingeling bbc main default (10), \\
     &       & Riss6 default\_DRAT (10), Riss6 noPP\_DRAT (10), COMiniSatPS Chandrasekhar DRUP drup (14), \\
     &       & glucosePLE default (14), Glucose\_nbSat default (17), tb\_glucose default (17), \\
     &       & cmsat5\_main2 default (17), MapleCOMSPS\_CHB\_DRUP CHB\_VSIDS\_drup (20), gulch default (20), \\
     &       & glucose\_hack\_kiel\_newScript main\_new (20), GHackCOMSPS\_DRUP ghack\_drup (22), \\
     &       & glueminisat-2.2.10-81-main maintrack (22), MapleGlucose default (24), Splatz 06v main default (25), \\
     &       & glue\_alt default (26), tc\_glucose default (26) \\
2    & 28    & Scavel\_SAT default (28) \\
3    & 29    & YalSAT 03r default (29) \\


==> tables/sat/main-crafted/sat2016_main_crafted_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
1    & 7   & tc\_glucose default (1), Riss6 noPP\_DRAT (2), Lingeling bbc main default (3), glucose\_hack\_kiel\_newScript main\_new (3), \\
     &     & MapleCOMSPS\_DRUP seq\_LRB\_VSIDS\_drup (5), tb\_glucose default (6), abcdSAT\_drup default (6), Riss6 default\_DRAT (8), \\
     &     & Beans And Eggs default (9), GHackCOMSPS\_DRUP ghack\_drup (9), COMiniSatPS Chandrasekhar DRUP drup (11), \\
     &     & glue\_alt default (11), MapleGlucose default (14) \\
2    & 17  & Splatz 06v main default (13), glucose default (15), MapleCOMSPS\_LRB\_DRUP LRB\_VSIDS\_drup (16), \\
     &     & Glucose\_nbSat default (17), MapleCOMSPS\_CHB\_DRUP CHB\_VSIDS\_drup (19), glueminisat-2.2.10-81-main maintrack (19), \\
     &     & glucosePLE default (19) \\
3    & 25  & MapleCMS default (21), cmsat5\_main2 default (21), Riss6 blackbox\_DRAT (23), cmsat5\_autotune2 default (24), \\
     &     & gulch default (24), Scavel\_SAT default (26), CHBR\_glucose default (27), CHBR\_glucose\_tuned default (27), \\
     &     & YalSAT 03r default (29) \\


==> tables/sat/nolimit/sat2016_nolimit_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 2    & BreakIDCOMiniSatPS default (1), Lingeling bbc notrace default (2), abcdSAT\_lim default (3) \\
     2 & 6.5    & MapleCMS default (4), tc\_glucose\_agile default (5), MapleCOMSPS\_no\_DRUP seq\_LRB\_VSIDS\_no\_drup (6), \\
       &         & Riss6 noPP (6), tb\_glucose\_agile default (8), COMiniSatPS Chandrasekhar no DRUP no\_drup (8) \\
     3 & 13    & MapleCOMSPS\_LRB\_no\_DRUP LRB\_VSIDS\_no\_drup (10), GHackCOMSPS\_no\_DRUP ghack (12), \\
       &          & MapleGlucose default (12), Riss6 default (12), Splatz 06v notrace default (14), \\
       &          & MapleCOMSPS\_CHB\_no\_DRUP CHB\_VSIDS\_no\_drup (15), glueminisat-2.2.10-81 default (16) \\
     4 & 18    & Riss6 blackbox (17), CHBR\_glucose\_agile default (18), CHBR\_glucose\_tuned\_agile default (18) \\
     5 & 20    & YalSAT 03r default (20) \\


==> tables/sat/random/sat2016_random_alt_rankings.tex <==
\textbf{Group} & \textbf{Fract. Rank} & \textbf{Solvers} \\
\midrule
     1 & 2.5    & dimetheus randomsat (1), CSCCSat default (2), DCCAlm default (3), polypower1.0 default (4) \\
     2 & 5.5    & polypower2.0 default (5), YalSAT 03r default (6) \\
     3 & 8    & stocBCD default (7), multi-sat default (8), cmsat5\_agile default (9) \\

